Examination of Community Sentiment Dynamics due to COVID-19 Pandemic: A Case Study from A State in Australia

The outbreak of the novel Coronavirus Disease 2019 (COVID-19) has caused unprecedented impacts to people's daily life around the world. Various measures and policies such as lockdown and social-distancing are implemented by governments to combat the disease during the pandemic period. These measures and policies as well as virus itself may cause different mental health issues to people such as depression, anxiety, sadness, etc. In this paper, we exploit the massive text data posted by Twitter users to analyse the sentiment dynamics of people living in the state of New South Wales (NSW) in Australia during the pandemic period. Different from the existing work that mostly focuses the country-level and static sentiment analysis, we analyse the sentiment dynamics at the fine-grained local government areas (LGAs). Based on the analysis of around 94 million tweets that posted by around 183 thousand users located at different LGAs in NSW in five months, we found that people in NSW showed an overall positive sentimental polarity and the COVID-19 pandemic decreased the overall positive sentimental polarity during the pandemic period. The fine-grained analysis of sentiment in LGAs found that despite the dominant positive sentiment most of days during the study period, some LGAs experienced significant sentiment changes from positive to negative. This study also analysed the sentimental dynamics delivered by the hot topics in Twitter such as government policies (e.g. the Australia's JobKeeper program, lockdown, social-distancing) as well as the focused social events (e.g. the Ruby Princess Cruise). The results showed that the policies and events did affect people's overall sentiment, and they affected people's overall sentiment differently at different stages.

==> NSW-measures.tex <==

https://www.theguardian.com/world/2020/may/02/australias-coronavirus-lockdown-the-first-50-days

25 January 2020:
Australia confirms its first case of the coronavirus — a Chinese national who flew into Melbourne on a flight from Guangzhou on January 19. Three more cases are identified in NSW and are held in isolation in hospital in Sydney. 

22 February 2020:
Twenty-four Australians were infected on the Diamond Princess cruise ship with eight being sent to Darwin for two weeks of quarantine.

27 February 2020:
The prime minister activated the Australian Health Sector Emergency Response Plan for Novel Coronavirus (COVID-19), stating that the rapid spread of the virus outside of China had prompted the government to elevate its response.

29 February 2020:
After a Queensland case of an infected person returning to Australia from Iran, the government extended the enforced quarantine to people who had been in Iran, requiring them to spend a fortnight in a third country before being allowed into Australia. There were 14 new cases in February, bringing the number of cases to 23. 
 
1 March:
Australia reported the first death from COVID-19: a 78-year-old Perth man, who was one of the passengers from the Diamond Princess, and who had been evacuated and was being treated in Western Australia.

8 March:
an 82-year-old man died becoming the second death at the Dorothy Henderson Lodge aged-care facility and the third death in the country. 

13 March: 
Peter Dutton the Home Affairs Minister for Australia was diagnosed in Queensland. 

15 March:
New South Wales schools have been told by the New South Wales Department of Education Secretary Mark Scott, to cancel all assemblies, excursions, travel and some events and conferences including arts and initiative events, as well as whole school sporting events and inter-school sporting events with three or more involved schools.

16 March, 
New South Wales Minister for Health and Medical Research Brad Hazzard announced that he was using his powers under Section 7 of the Public Health Act 2010 to immediately and indefinitely cancel all public events with more than 500 attendees. The order is enforceable by NSW Police and violations of the order carry a prison term of six months, an AUD11,000 fine, or both.

18 March
a human biosecurity emergency was declared by the Governor-General, David Hurley, under Section 475 of the Biosecurity Act 2015.

18 March
The cruise ship Ovation of the Seas docked in Sydney on 18 March and discharged about 3,500 passengers. 79 passengers had tested positively for the virus by 1 April.

19 March
The cruise ship Ruby Princess discharged 2,700 passengers in Sydney on 19 March. It was announced on 20 March that three of 13 passengers tested positive for the coronavirus. New South Wales health authorities asked all passengers to go into self-isolation.

19 March, 
Qantas confirmed it would suspend about 60 percent of domestic flights, put two thirds of its employees on leave, suspend all international flights and ground more than 150 of its aircraft from the end of March until at least 31 May 2020

20 March,
Even though there was a ban on gatherings of more than 500 people, huge crowds flocked to the popular Bondi Beach and other beaches across Sydney on Friday 20 March. 

22 March, 
the government announced a second stimulus package of AUD 66bn, increasing the amount of total financial package offered to AUD 89bn. This included several new measures; most notably a doubling of income support and relaxed eligibility criteria for individuals on Jobseeker's allowance and grants of up to AUD 100,000 for small and medium-sized businesses.

24 March 
one passenger from Ruby Princess had died and 133 on the ship had tested positive. On 28 March 284 passengers had tested positive.

25 March 
the National COVID-19 Coordination Commission (NCCC) was established by the Prime Minister, as a strategic advisory body for the national response to the pandemic.

30 March, 
at least 440 passengers from Ruby Princess had tested positive for the virus. As of 31 March 2020, five of them had died,

31 March 2020
Official lockdown in NSW
The NSW Government has now imposed a lock-down on the people of NSW, with the aim of reducing the spread of COVID-19. The arrangements are set out in the Public Health (COVID-19 Restrictions on Gathering and Movement) Order 2020 published late last night, only a short time before it came into effect this morning (on 31 March 2020).

5 April, 
New South Wales Police launched a criminal investigation into whether the operator of Ruby Princess, Carnival Australia, broke the Biosecurity Act 2015 (Cwth) and New South Wales state laws, by deliberately concealing COVID-19 cases.



15 May 2020
NSW to ease lockdown restrictions from Friday 15 May, the following is allowed:

    public gatherings of up to 10 people
    food and drink premises can open, but only to seat a maximum of 10 customers at any one time – this includes cafes and restaurants, a restaurant within a registered club or pub, or a cellar door that serves food
    up to 5 visitors may visit another household at any one time
    weddings can have up to 10 guests plus the people conducting or assisting in the conduct of the service, a photographer, a videographer, and the couple
    indoor funerals and memorial services can have up to 20 mourners and outdoor funerals up to 30 mourners
    religious gatherings and places of worship can have up to 10 worshippers
    outdoor playground and exercise equipment can be used with caution
    outdoor pools can open with restrictions.

